MANETs monitoring with a distributed hybrid architecture

Monitoring techniques have been deeply studied in wired networks using gossip and hierarchical approaches. However, when applied to a MANET, several problematics arise. We present a hybrid distributed monitoring architecture for MANETs. We get inspired of gossip-based and hierarchical-based algorithms for query dissemination and data aggregation. We define gossip-based mechanisms that help our virtual hierarchical topology to complete the data aggregation, and then ensure the stability and robustness of our approach in dynamic environments. We propose a fully distributed monitoring protocol that ease the nodes communications. We evaluate our approach by using NS3 and Docker.

==> 02_preliminaries/preliminaries.tex <==
\section{Preliminaries} \label{preliminaries}

%Network monitoring is an extensive field of interest.
%It refers to measuring and collecting information about a property in the network.
%There are actually multiple definitions but it depends on the context.
%We will present the basic terms for the reader to understand the following sections.

%\subsection{Network Monitoring}

Network monitoring can be described as \say{A number of observers making observations, and wish to work together to compute a function of the combination of all their observations} \cite{cormode2013continuous}. % (definition from \cite{cormode2013continuous}). 
%The observers in our case are the nodes in a MANET.
The goal is that all the nodes in the network compute a value $t\mapsto f(t)$ [$\mathbb{R}^{+*}\rightarrow X$, $X$ being the domain targeted by $f$] in a given instant of time $t$ in a collaborative way.
%The function $t\mapsto f(t)$ [$\mathbb{R}^{+*}\rightarrow X$, $X$ being the domain targeted by $f$],
For our purposes, $f$ is a linear and non-complex function (e.g., the average CPU).%, %average RAM usage, 
%or any other nominal value.
%The computation, communication, aggregation and any other mechanism involved in the monitoring process of the observations will occur in a time $\tau$, assuming that $\tau > 0$.
%Given this definition, we can imply that every node in the network is a point of observation of a property.
%These observations need to be analyzed in a network scale to be able to determine the health and state of the overall network over a given property.
%It is important to mention t hat the monitoring process can be triggered by an event or by a periodic polling.
% , for example a new value of a monitored property or a query to compute the global view of a property.
% Or it can also be triggered by a periodic polling.

The monitoring process can be classified in centralized and decentralized \cite{battat2014monitoring}. %, as studied by \cite{battat2014monitoring}. 
The centralized approach \cite{cormode2013continuous} % as stated by \cite{cormode2013continuous}, 
is when all the nodes report their observations to a central entity (centralizer or coordinator).
The decentralized one considers networks with no centralizer. The main current decentralized approaches are gossip and hierarchical \cite{stingl2012benchmarking}.
%As stated in \cite{stingl2012benchmarking}, %the more noticeable, for the time being, 
%the main current decentralized approaches are gossip and hierarchical.

% \subsection{Types of Monitoring}

% The classification of the monitoring process has been studied in \cite{battat2014monitoring}.
% For the purposes of this paper, we will consider two major types: centralized and decentralized.
% The centralized type of monitoring, as stated by \cite{cormode2013continuous}, is when all the nodes report their observations to a central entity, named centralizer or coordinator.
% This entity will process all the observations from all nodes in order to reach a global view of this property of the network.
% This approach is the most common scenario and it can be found multiple articles in the literature that analyze and optimize it.
%The decentralized type of monitoring, 
% The decentralized approach, the opposite of the previously defined approach, deals with networks where there is no centralizer entity.
% This implies that the network by itself needs to achieve a global view of a property of the network.
% The preferred approach is to get the global view of a property of the network, and then disseminate it through the entire network to assure that is available to all the network.
%As stated by \cite{stingl2012benchmarking}, the more noticeable, for the time being, approaches are gossip and hierarchical.
%\subsubsection{Gossip-based approaches}
The gossip approaches are based on the gossip or epidemic algorithms.
Gossip algorithms rely on selecting, from a set of reachable nodes, a random or a specific node (depending on the algorithm) to forward the data packet \cite{chakchouk2015survey}. 
%There are multiple types of gossip techniques, a more detailed study can be found in \cite{chakchouk2015survey}.
%In this publication, the focus is on routing protocols.
%It explains how gossip based protocols implement through different techniques and properties their goals.
% This is achieved by using different properties according to their purpose.
% For example energy efficient gossip based protocols inter change information about their batteries to be more efficient.
% Or probabilistic gossip based protocols that use the probabilities of meeting a node to their advantage.
% A general assumption in this kind of protocols, is that the nodes requires to be synchronized.
Epidemic algorithms try to forward the packet not only to one but to multiple nodes. 
%And they also are considered the same or a subcategory of the gossip algorithms.
%Flooding is the most common and simple algorithm for epidemic algorithms.
Gossip based monitoring algorithms have the advantage of being highly stable and perform better in increasing dynamic networks. 
%But also have the disadvantage of generating a lot of traffic and under certain scenarios it requires more time to compute a value.
%\subsubsection{Hierarchical-based approaches}
In the hierarchical approaches, the leaf nodes communicate recursively the values with their parent node. 
%This approach is using a tree structure.
%In which the leaf nodes communicate recursively the values with their parent node.
%This is done recursively until it reaches the root node of the hierarchy.
%These approaches consider a mechanism of either pulling data or pushing data with their nearby nodes.
For a hierarchical algorithm to work over a network, it will need to build the topology before being able to monitor.
%The advantages %of hierarchical based monitoring algorithms 
%are that they are able to quickly converge the monitoring of a property and producing less traffic.
%The disadvantages are that they are prone to errors in the event of a crash in the network. 
%This means that it does not perform efficiently in a highly dynamic environment.

==> 03_methods/timeline.tex <==
\begin{figure}
\centering

\scalebox{0.95}{%

\begin{tikzpicture}[node distance=2cm,auto,>=stealth']
  \node[] (node0) {node0};
  \node[right = of node0] (node11) {node1.1};
  \node[right = of node11] (node21) {node2.1};
  \node[below of=node0, node distance=4cm] (node0_ground) {};
  \node[below of=node11, node distance=4cm] (node11_ground) {};
  \node[below of=node21, node distance=4cm] (node21_ground) {};
  %
  \draw (node21) -- (node21_ground);
  \draw (node11) -- (node11_ground);
  \draw (node0) -- (node0_ground);
  \draw[<-] ($(node11)!0.25!(node11_ground)$) -- node[above,scale=0.7,midway]{SND Query} ($(node0)!0.25!(node0_ground)$);

  \draw[->] ($(node11)!0.40!(node11_ground)$) -- node[above,scale=0.7,midway]{SND Query} ($(node0)!0.40!(node0_ground)$);
  \draw[->] ($(node11)!0.40!(node11_ground)$) -- node[above,scale=0.7,midway]{SND Query} ($(node21)!0.40!(node21_ground)$);
  \draw[-] ($(node0)!0.40!(node0_ground)$) -- node[left,scale=0.7,midway]{acc(ACK\_IP)} ($(node0)!0.40!(node0_ground)$);

  \draw[-] ($(node21)!0.50!(node21_ground)$) -- node[right,scale=0.7,midway]{edgeNode()} ($(node21)!0.50!(node21_ground)$);

  \draw[->] ($(node21)!0.60!(node21_ground)$) -- node[above,scale=0.7,midway]{SND Aggregate} ($(node11)!0.60!(node11_ground)$);

  \draw[->] ($(node11)!0.75!(node11_ground)$) -- node[above,scale=0.7,midway]{SND AggregateACK} ($(node21)!0.75!(node21_ground)$);
  \draw[->] ($(node11)!0.75!(node11_ground)$) -- node[above,scale=0.7,midway]{SND Aggregate} ($(node0)!0.75!(node0_ground)$);

  \draw[->] ($(node0)!0.90!(node0_ground)$) -- node[above,scale=0.7,midway]{SND AggregateACK} ($(node11)!0.90!(node11_ground)$);

  \draw[-] ($(node0)!0.95!(node0_ground)$) -- node[left,scale=0.7,midway]{done()} ($(node0)!0.95!(node0_ground)$);
\end{tikzpicture}

}

\caption{Timeline view of the events between node0, node11 and node21 in the example presented} \label{fig:timeline}
\end{figure}

==> 05_discussion/discussion.tex <==
\section{Future Work} \label{futurework}

% We have several perspectives for our. 
We intend to study the selection of the root node.
% So far we have focused on how the approach works for a time window.
% The intention of doing this, was to define in a concise way the VHT (virtual hierarchical tree).
%But we need some mechanisms and proposals on how to select the main node.
It could be based on location, energy, computing power and other parameters.
It could also be an autonomous process, proactively or reactively, or a manual process. %that needs to be performed by an operator.

Besides we plan to introduce the mobility support and enhance the testbeds to this specific cases.
We will target diverse distributed monitored environment such as urban networks. 
%want to enhance the testing  our approach.
%We plan to use robust tools as the emulation tool Dockemu \cite{to2015dockemu} used in \cite{to2015spanning}.
We will be looking for specific metrics under different scenarios in a scalable way.
%In particular, we expect to assess the performance in terms of convergence of communication packets with a high node speed.
%We believe that the proposal is very promising, but there are multiple areas to define and enhance.

% Another area of interest, is to handle the monitored property after the time window.
% So far this process is calculated using a hybrid algorithm, but it could be stored in all nodes or in a coordinator.
% We intend to analyze this options into our proposal, to maximize the options and scenarios to cover with our approach.

Lastly we intent to analyze and take into consideration more complex functions.
We are interested in monitoring the interoperability within a MANET.
For this we need to define an optimal solution to propagate a more complex function through our query mechanism.
%This requires to analyze multiple interoperability approaches to provide a proposal for monitoring this process.
To monitor interoperability we believe that it is needed to analyze not all observation points in the network, but more specifically a subset of observation points.
